Machine Learning Explanations to Prevent Overtrust in Fake News Detection

Combating fake news and misinformation propagation is a challenging task in the post-truth era. News feed and search algorithms could potentially lead to unintentional large-scale propagation of false and fabricated information with users being exposed to algorithmically selected false content. Our research investigates the effects of an Explainable AI assistant embedded in news review platforms for combating the propagation of fake news. We design a news reviewing and sharing interface, create a dataset of news stories, and train four interpretable fake news detection algorithms to study the effects of algorithmic transparency on end-users. We present evaluation results and analysis from multiple controlled crowdsourced studies. For a deeper understanding of Explainable AI systems, we discuss interactions between user engagement, mental model, trust, and performance measures in the process of explaining. The study results indicate that explanations helped participants to build appropriate mental models of the intelligent assistants in different conditions and adjust their trust accordingly for model limitations.

==> sections/model_old_.tex <==



% --------------- 2020 version ---------------

We implement an ensemble of four classifiers for fake news detection generating different types of explanations.
We obtain final prediction score through averaged ensemble results with \emph{73.65\%} detection accuracy.
We briefly review details of each model in the following. %  and how each model is used in in next sections.

Our first model is a Bi-LSTM network with an additional self-attention layer to extract attention scores for instance explanations.
We use Word2Vec\cite{mikolov2013distributed} to embed each word into an embedding vector before feeding into the network. 
Final prediction is conducted with weighted attention scores.
This model is only trained with the news headlines which is part of our data.
And the generated explanations are in form of salient word heatmap for news headlines. 
We compare this model with several baselines, including CNN, RNN, LSTM and RCNN, and find out that our model can outperform those baseline model significantly. In particular, CNN achieves 65.42\% accuracy, RNN achieves 63.27\%, LSTM achieves 65.39\% and RCNN achieves 66.17\%, while our first Bi-LSTM + Self-Attention model can achieve \emph{72.00\%} accuracy performance in detection fake news claims. 
% Detection accuracy for this model is 72\%.



The Second model performs fake news detection based on both claim representation and article set representation. 
The article set representation is constructed using hierarchical attention at sentence level and article level.
Using this design we can get 1) an importance score for each article and 2) select top-3 important sentences in each article using attention weighs. 
Finally, a weighted sum is performed over all articles to build the article representation, which is combined with the claim representation to form the final vector representation for claim classification. 
Specifically, the sentence embedding is achieved by averaging all the word embeddings inside the sentence. We use a Bi-LSTM network and an attention network to learn the representation of a claim. A Bi-LSTM captures both the previous time-steps and the future time-steps via forward and backward states respectively. Correspondingly, there are two hidden states that capture past and future information that are concatenated to form the final output. A single-layer attention is imposed over the output of the Bi-LSTM to aggregate information from important words inside the claim. The query vector of the attention mechanism is learned and represents the overall context of the claim. An importance weight for each word is achieved by attending the query to each word embedding. Finally, a weighed sum is performed to construct the vector representation of the claim. It is important to consider the relevance of each article with respect to the claim. We score each article and select the most important sentences in each article. We use the hierarchical attention network (HAN)~\cite{yang2016hierarchical} to help our model focus on the salient sentences and articles at two levels. Each sentence representation of an input article is generated by taking an average of the word embeddings of all the words therein. BiLSTM is firstly used to capture long dependencies before the attention is performed. For both levels, we use claim representation as query to attend sentence embeddings and article embeddings.
Current classification accuracy on the test set is 76.04\%. Our proposed model achieves a trade-off between the performance and interpretation. For some claims, the model tends to select the first several articles based on google search, which makes sense for the top ranked articles contain highly-related phrases with the claims.
% Attention weights are achieved and serve as importance scores for sentences and articles. 
% The Accuracy: 76.04%

For the third model, We use a knowledge distillation approach~\cite{hinton2015distilling} to approximate a deep architecture (teacher) with a random forest (student) model for our third fake news detector.
With the mimic learning framework, we can leverage the performance of deep model and analyze the attribute importance of news claims, article, and news sources for each prediction. 
For the overall training process, it is a two step training process. 
First, we train teacher model and use it train student model at second stage. 
For teacher model, we use Glove Wikipedia 6B word embeddings(100d)~\cite{pennington2014glove}, Adam optimizer with dropout, BiLSTM of size 128. We randomly initialize the source embeddings of claim and article with a length 8 vector and are learnt on fly. 
For student model, we train with 60 trees XGBoost~\cite{chen2016xgboost} model. 
Further, through the constructed forest, end-users could exactly know what happened in the prediction model, which provides users an overall transparency towards the model itself. 
When evaluated on the test set, our third model has 72.08\% accuracy. The model level importance of 4 input attributes from student model are Article source(42\%), Claim source(12\%), Article(26\%), Claim(20\%). This also implies that student model is using source of article as main criteria for doing classification. 
% Accuracy 72.08\%

Our last model considers the context of the claim via word embedding as well as the articles captured by a bidirectional LSTM (BiLSTM) module. 
We use an attention mechanism to focus on parts of the articles according to their relevance to the claim. 
Our method then aggregates all the information about the claim, article contexts, and attention weights, in order to assess the claim credibility. 
Attention mechanism is utilized in our model to generate user-comprehensible explanations, making credibility verdicts transparent and interpretable.
To create an attention-focused representation of the article that takes into account both the claim and the article language, we calculate a weighted average of the hidden state representation based on the attention score corresponding to all the article tokens~\cite{kumar2019attentional}. Finally, in order to generate an overall credibility label for the classification task, the final representation is processed using the final fully connected layer.
Suppose each claim has $m$ reporting articles. Once we have the credibility score for each article from our model, we average those scores to generate the overall credibility score for the claim. This aggregation is done after the model has been trained. The current accuracy on Snopes test set is 65.6\% if using 10 attention vectors, 68.3\% if using 30 attention vectors, and 69.8\% if using 50 attention vectors.
% Accuracy 69.80\%

As a decision point for trade-offs between clarity and faithfulness of explanations, we perform simple post processing of model explanations to remove very small features scores in word attention heatmap and normalization of attributions scores between articles. 



==> sections/quad-figure.tex <==

\begin{figure}
\captionsetup[subfigure]{justification=centering}
\centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1.05\columnwidth]{figures/risk-TPR-mix-10.pdf}
        \caption{CIFAR-10 $D^{in}$ }
    \end{subfigure}
    %   \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1.05\columnwidth]{figures/risk-TPR-mix-100.pdf} % figures/cifar100_ROC+ODIN+OE.pdf
        \caption{CIFAR-100 $D^{in}$ }
    \end{subfigure}
\captionsetup[subfigure]{justification=centering}
    \centering
   \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1.05\columnwidth]{figures/risk-cov-mix-10.pdf}
        \caption{CIFAR-10 $D^{in}$ }
    \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1.05\columnwidth]{figures/risk-cov-mix-100.pdf} 
        \caption{CIFAR-100 $D^{in}$ }
    \end{subfigure}
  \caption{Comparison between the Baseline, OE, and our method's total misclassificaiton error rate~\textbf{(Top)} for CIFAR-10 and CIFAR-100 experiments at different OOD detection TPR. 
  $D_{test}^{out}$ set is an equal mix of five different test sets.
  Our method shows the highest test set coverage~\textbf{(Bottom)} at all classification error rate.}
  \label{fig:quad-results}
\end{figure}


==> sections/qualitative_old_.tex <==


\subsection{Qualitative Feedback}

Participants qualitative feedback in the post-study survey reflects their reasoning about AI assistant and provides justifications for our quantitative results. 
We asked participants three descriptive questions regarding their mental model of AI assistant reasoning (``\textit{How do you describe this AI's reasoning to find fake news?}''), AI assistant limitations (``\textit{In your opinion, what are the biggest limitations of this AI fake news detector?}''), and their task strategy (``\textit{What was your strategy for selecting true news stories?}''). 
% and how they could improve their strategy (``What additional information or explanations could have helped you to make your decisions?'').
% Two authors reviewed and coded participants response for each question in three iterations of open coding (individually) and discussion (in group).  --- not ready ---
The mean participant response length was 77.8 words (range = [338, 28], SD = 46.4) for all descriptive response forms. % of each participant. 

% \eric{maybe less important paragraph}
Looking at participant feedback regarding their strategies in selecting news articles shows an overall theme of uncertainty and subjectivity in participants decision-making for reviewing news stories. 
For examples participants mentioned ``\textit{my own intuition}'' and ``\textit{my common sense}'' as well as ``\textit{by how feasible the headlines seemed}'' as parts of their strategies. 
Some participants also mentioned the inherit complexity in recognizing fake news.
For example, one said ``\textit{Well it can never know for sure if it's fake or not}''.
% Another feedback trend was to request more news meta-data such as ``\textit{trends in social media}'' and ``\textit{[human] fact checker opinions on all articles}''. 
This qualitative feedback reinforces that news review and fact checking are difficult tasks involving uncertainty for users.

% \eric{any percentage or quantification of such appropriate comments relative to incorrect mental model responses?} -> unfortunately, no.
Regarding participant mental models of AI assistants, we observed that explanations clearly affected their understanding of AI reasoning. %  although same models are used in all conditions, 
Participants in the \textit{XAI-attention} group pointed out the importance of keywords in the news; example comments include ``\textit{I think it looked for certain key words}'' and 
% \begin{quote}
``\textit{The AI compares relevant phrases in the headline to relevant keywords in the supporting stories.}''
% \end{quote}
However, participants in the \textit{XAI-attribution} group mentioned related articles and their sources as key features in AI reasoning. 
For example, one participant in the \textit{XAI-attribution} group commented ``\textit{It tries to pull related articles from the web to prove or disprove the headline}'', and another participant indicated the use of ``\textit{The origin of the info. i.e the site it came from.} % Scopes Wall Street Journal etc}''. % ``It was based on amount of article's that had words similar to the headline''

We also found interesting feedback on participants' subjective opinions on the limitations of the AI assistant. 
We saw a clear theme in responses to the need for common sense to distinguish fake and true news. 
From many participants in the \textit{AI assistant} and \textit{XAI assistant} conditions, we received comments such as ``\textit{it doesn't have human judgment}'', ``\textit{I guess they will not see common sense}'', and ``\textit{The AI doesn't have the experience that a real person has in dealing with the fake news out there.}''. 

% The first participant appears to be ... which is understandable. The second ... 

Additionally, some participants expressed concern about AI ability in understanding the context of real news or recognizing sarcasm. 
For instance, one said ``\textit{I think it can't detect sarcasm satire or parody so it has some limitations}'' and another mentioned that ``\textit{The AI isn't able to understand the context of the text. It's not able to actually understand the story or [its] plausibility.}''. % , as well as:

% \begin{quote}
% ``\textit{It can't seem to discern between junk news and the real deal. It can't discern that a site is biased. It could pull the keywords that's for certain but any site could have the keywords. There's more to it than that and it can't do it.}''
% \end{quote}


\noindent Other participants mentioned the limitations in related articles that the AI assistant was relying on, giving comments such as: 

\begin{quote}
``\textit{In multiple instances the AI seemed to struggle to find relevant information as many of the provided articles were tweets or Facebook posts that lacked any information at all relevant or otherwise. That made me question how the AI arrived at its judgment.}''
\end{quote}


Overall, qualitative results align with our quantitative findings, and participants in the \textit{XAI assistant} conditions could described model reasoning and weaknesses. %  in comparison to the \textit{AI assistant} condition. 
% and opens new directions to improve AI assistant design for end-users.

% Overall, participants in the \textit{XAI assistant} conditions better understood model reasoning and weaknesses in comparison to the \textit{AI assistant} condition.
% The qualitative results align with the previously presented quantitative findings. % and opens new directions to improve AI assistant design for end-users.

==> sections/results-fig-mental.tex <==
\begin{figure}
\captionsetup[subfigure]{justification=centering}
\centering
   \begin{subfigure}[b]{0.47\columnwidth}
        \includegraphics[width=1.0\columnwidth]{figures/mental-1.PNG}
        \caption{User Prediction Accuracy}
    \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        % \includegraphics[width=1.0\columnwidth]{figures/mental-2-new.PNG}
        % \caption{Task Cognitive Load}
    \end{subfigure}
  \caption{Evaluation of user (a) mental model through guessing model output and 
%   (b) cognitive load \TODO{time per news review} through news review time for AI 
  Assistant, and three XAI Assistant conditions. \TODO{remove this figure? keep it?}}
  \label{fig:mental}
\end{figure}



==> sections/results-fig-performance.tex <==

\begin{figure}
\captionsetup[subfigure]{justification=centering}
\centering
   \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{figures/performance.png}
        \caption{Credibility Score for Shared True News}
    \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{figures/performance-2.PNG}
        \caption{Incredibility Score for Reported Fake News}
    \end{subfigure}
  \caption{User performance measures for Baseline, AI Assistant, and XAI Assistant conditions. \eric{is there an appropriate term that applies to both instead of the credibility-incredibility pair. something like "correct identification score"?} \TODO{candidate to be removed} \TODO{add figure references in the section X}}
  \label{fig:performance}
\end{figure}



==> sections/results_old_.tex <==
% \section{Evaluation Results}
\section{Study Results}
We first review the participant information and then the study results in the following subsections. We recruited 180 participants in our between-subject crowdsourced study which 47\% were female, with 37.8\% between 30-39 years old, 30.3\% between 40-59 years old, 15.9\% between 20-29 years old, and 3\% between 50-59 years old; 51\% had a bachelor's degree, 23\% had a college degree less than bachelor, 14\% had graduate school degree, 14\% had highschool education, and 1\% had less than highschool education. 

% >> add the new 30 participants and update
% >> remove time outliers and update
Total 94.53 hours study time was recorded for 180 participants on averaged payment of \$10.68/hour. Average news review and selection duration was 30.5 minutes (range = [132,2.96] with SD = 20.9); average number of user clicks was 162 clicks (range = [410, 35], SD = 77.2); average character count on free response forms was 77.8 characters (range = [338, 28], SD = 46.4) for each study.



% \subsection{AI Assistant Usefulness:}
% Before analyzing study data for main research questions, we were interested if explanations provided in XAI assistant conditions...

% \noindent \textbf{H1: Users will engage more with explanations that are helpful for their task. }

% Our objective measure for AI/XAI usefulness was user rate of checking AI/XAI assistant prediction when sharing or reporting news (M9).



\subsection{News Credibility:}
% \subsection{News Credibility:}

Analysis of our three performance measures shows averaged credibility of shared news is the highest in XAI-all condition and is lowest on no-AI conditions. The credibility of the original input mix of news stories for users were set on 50\% and our AI/XAI assistant was set of 66.6\% detection accuracy. We provided charts for results and performed ANOVA test followed by Tukey’s post-hoc test for all measures. 


\noindent \textbf{H2: Users can share more true news stories with the help of XAI algorithm.}

Our two first performance measures is defined based on sharing true news (primary task).


\textit{Results:} Figure 4 shows the box-plot chart of participants’ shared newsfeed credibility scores for the five conditions. Average credibility score is higher than the original news feed (50\% credibility) in all groups. User shared news lists had higher (1\%-6\%) credibility than AI and XAI conditions, but 0.3\% less on no-AI condition. The data met the assumptions for parametric testing for all groups with validation checks passing for data normality (Shapiro-wilk test) and homogeneity of variances (Levene's test) tests. A significant effect was observed by an ANOVA test with F(4, 121) = 2.741 and p = 0.032 for the newsfeed credibility measure. However, the Tukey’s post-hoc test did not show significant difference between groups. 

\textbf{H3: Users can report more fake stories with the help of XAI algorithm. }

We measure credibility of 12 shared true news and incredibility (1.0 - credibility) of all reported fake news as performance measures.

\textit{Results:} 
Figure 5 shows a box-plot chart of reported fake news incredibility (1.0-credibility score) for five groups. The XAI-all group has the highest average incredibility of reported fake news stories.  However, explanation types or AI assistant did not significantly affect user performance [F(4,122) = 1.441, p = 0.225] when measuring incredibility of reported fake news. This is possibly because of the fact that reporting fake news was not the user’s primary task during the study. 

% \noindent \textbf{H4: Users can perform their tasks faster with the help XAI algorithm.}

% We also take total duration (minutes) of news review and selection duration (excluding survey and instruction pages) as our third performance measure (M3). 

% \textit{Results:} 
% Figure 6 shows a box-plot chart of task duration (instruction and survey excluded) for five groups. AI and different XAI assistants did not significantly affect user performance (F(4,118) = 0.712, p = 0.585) when measuring time as a performance measure. This is possibly because we allowed participants to spend as much time as they needed (compensated up to 1 hour) on the task to share 12 true news stories. Data normality (Shapiro-wilk test) and homogeneity of variances (Levene's test) tests were passed  for all four groups.

\input{sections/results-fig.tex}


\subsection{User Mental Model:}

Analysis of our mental measures show an overall advantage of XAI-all and XAI-attribution over XAI-attention and AI conditions. We review results for two quantitative and two qualitative mental model evaluation results.

\noindent \textbf{H5: Users can predict model output more accurately if they have an appropriate understanding of the model from explanations.}
Our primary measure for quantitative evaluation of mental model is user accuracy in predicting of model output (M4). We ask pop-up questions from participants to guess “what would the AI fake news detector predict for this news story?” for the last third of the study. 

\textit{Results:} 
Figure 7 shows a box-plot for user prediction task results from four groups. User prediction task accuracy was best in the XAI-attribute group and the worst in the AI group. The data passed parametric tests for normality (Shapiro-wilk test) and homogeneity of variances (Levene's test). An ANOVA test detected a significant main effect with F(3,89) = 2.926 and p = 0.038 for user accuracy of predicting model output. However, the Tukey’s post-hoc test did not show significant difference between groups.



\noindent \textbf{H6: Users can better understand model reasoning and find model weaknesses if they have an appropriate mental model the algorithm.}
Our qualitative evaluation is focused on users identifying model reasoning (M6) and weaknesses (M7). We use two free response forms at the end of study to collect user feedback regarding (Q1: “How do you describe this AI's reasoning to find fake news?”) and (Q2: “In your opinion, what are the biggest limitations of this AI fake news detector?”). We review results and average character count from user responses for each question on Section 5-3

\subsubsection{Qualitative Results:}
Detailed analysis results for qualitative data is not ready at the date of this report.



\subsection{User Trust on AI Assistant:}
Analysis of our trust measures show participants had higher trust on XAI-attribute and XAI-all assistants compared to XAI-attention and AI assistants. 

\noindent \textbf{H6: Users’ perceived accuracy is higher with more trust in the XAI system. }
Our last measure for user trust is users’ perceived model accuracy (M12) at the end of study. We asked users to set a continuous slider bar to indicate their understanding of AI accuracy (“What was the accuracy of the AI fake news detection?”).

\textit{Results:}
Figure 13 shows a box-plot chart of user perceived accuracy of AI/XAI models at the end of study from four groups. Average AI/XAI accuracy was set on 66\% based on one misdetected instance (false positive or false negative) for every two correct detection instances (true positive and true negative) in the user list of news story. However, results show in all conditions users guessed lower model accuracy for the AI/XAI algorithm. 
The study did not detect a significant effect between groups for their perceived accuracy of AI/XAI assistants. However, user trust in the XAI-attribution condition (M = 59.24\%) was slightly higher than the XAI-all (M = 51.05\%), XAI-attention (M = 51.73\%), and AI (M = 52.70\%) conditions. Data normality (Shapiro-wilk test) and homogeneity of variances (Levene's test) tests were passed  for all four groups except XAI-attribution. 


\noindent \textbf{H7: Users will accept more XAI assistant suggestions with higher trust to the system. }
Our objective measure for user reliance on AI/XAI assistant was user rate of agreeing with the AI prediction when share or reporting news (M11). 

\textit{Results:}
Figure 12 shows a box-plot chart of user compliance/agreement rate with the AI/XAI assistant from the four groups. User compliance rate is measured regardless of news credibility, however, higher compliance rate in XAI-all resulted in higher news credibility score in users shared news.
After removing one outlier data point, the data passed checks for normality (Shapiro-wilk test) and homogeneity of variances (Levene's test) tests. We observed a significant main effect in an ANOVA test with F(3,115) = 9.965 and p < 0.001 for engagement with AI prediction output. A Tukey post-hoc test showed users had significantly lower compliance with the AI assistant in the XAI-attention group compared in the AI group, XAI-attribution group, and XAI-all group (p < 0.001 for all pairwise comparisons). 
 
 
 
\noindent \textbf{H8: User trust in the system changes over time representing transitions between under trust, overtrust, and appropriate trust.}


\textit{Results:}
We also measured user perceived accuracy of AI/XAI algorithm twice during the study to evaluation user trust changes over time. Figure 14 shows the box-plot chart of shifts in user perceived accuracy over time between our first and last measurements. 

The analysis did not detect a significant effect between groups for shifts in perceived accuracy of AI/XAI assistants. However, user trust changes over time on XAI-attribution condition (M = 3.50\%) was slightly higher than XAI-all (M = 2.03\%) and XAI-attention (M = 1.35\%). User trust in AI condition was negative (M = -0.40\% which indicates that participants lost trust over time between our first and last measurements.

